Automatic Unit Test Generation for Deep Learning Frameworks based on API Knowledge

Many automatic unit test generation tools that can generate unit test cases with high coverage over a program have been proposed. However, most of these tools are ineffective on deep learning (DL) frameworks due to the fact that many of deep learning APIs expect inputs that follow specific API knowledge. To fill this gap, we propose MUTester to generate unit test cases for APIs of deep learning frameworks by leveraging the API constraints mined from the corresponding API documentation and the API usage patterns mined from code fragments in Stack Overflow (SO). Particularly, we first propose a set of 18 rules for mining API constraints from the API documents. We then use the frequent itemset mining technique to mine the API usage patterns from a large corpus of machine learning API related code fragments collected from SO. Finally, we use the above two types of API knowledge to guide the test generation of existing test generators for deep learning frameworks. To evaluate the performance of MUTester, we first collect 1,971 APIs from four widely-used deep learning frameworks (i.e., Scikit-learn, PyTorch, TensorFlow, and CNTK) and for each API, we further extract its API knowledge, i.e., API constraints and API usage. Given an API, MUTester combines its API knowledge with existing test generators (e.g., search-based test generator PyEvosuite and random test generator PyRandoop) to generate test cases to test the API. Results of our experiment show that MUTester can significantly improve the corresponding test generation methods and the improvement in code coverage is 15.7% to 27.0% on average. In addition, it can help reduce around 19.0% of invalid tests generated by the existing test generators. Our user study with 16 developers further demonstrates the practicality of MUTester in generating test cases for deep learning frameworks.

==> figure/API_with_parameters.tex <==


\begin{figure}[h]
 \begin{subfigure}{0.5\textwidth}
\includegraphics[width=\columnwidth]{figure/API_with_parameters.PNG}
\caption{API Document of Sklearn.cluster.KMeans.fit}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
 \includegraphics[width=\columnwidth]{figure/ei_pr.jpg}
\caption{Extracted Information from API documents with their respective parametric sentence rules used for mining.}
\label{fig:subim2}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=\columnwidth]{figure/Output Table.png}
\caption{Extracted Constraints of Parameters \song{(b) is barely readable}}
\label{fig:subim2}
\end{subfigure}

\caption{API Document Mining}
\label{fig:image2}
\end{figure}


==> figure/SO.tex <==
\begin{figure}[t!]
    \centering
      \includegraphics[width=\columnwidth]{figure/SO_mining.png}
    \caption{Overview of API Usage Pattern Mining from SO.}
    %\nima{The figure has low resolution. The text are very difficult to read.}
   \label{fig:SO}
\end{figure}


==> figure/boxplot/comparison_AUC.tex <==
\begin{figure*}[th!]
\centering
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/boxplot/proprietary.tex}
\vspace{-0.2in}
\caption{{\companyX}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/boxplot/qt.tex}
\vspace{-0.2in}
\caption{Qt}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/boxplot/android.tex}
\vspace{-0.2in}
\caption{Android}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/boxplot/openstack.tex}
\vspace{-0.2in}
\caption{OpenStack}
%\vspace{-0.1in}
\end{subfigure}\hfill

\vspace{-0.1in}
\caption{ \small
Comparison of perdition performance (AUC) between the specific 
models and the general models. 
The model with a prefix ``G'' means using the trained general model to predict 
changes with a particular intent.  
``b'' represents `Bug Fix',
``re'' represents `Resource',
``f'' represents  `Feature',
``t'' represents `Test', 
``r'' represents `Refactor', 
``m'' represents  `Merge', 
``d'' represents  `Deprecate', 
and ``o'' represents  `Others'. 
For example \textbf{G-b} means using the trained general model 
to predict changes with the `Bug Fix' intent.
\textbf{S-b} is the specific model  
trained and evaluated on changes with the `Bug Fix' intent.
}
\label{fig:comparison}
\vspace{-0.1in}
\end{figure*}
%\vspace{-0.1in}


==> figure/boxplot/openstack.tex <==
\scalebox{0.55}{
\begin{tikzpicture}
\pgfplotsset{
	   boxplot/every whisker/.style={thick,solid,black},
	   boxplot/every median/.style={very thick,solid,black},
	   %boxplot/every box/.style={very thick,solid,draw=songcolor},
}
\begin{axis}[
xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15},
%xticklabels={G-bug,S-bug,G-resource,S-resource,G-feature,S-feature,
%G-test,S-test,G-refactoring,S-refactoring,G-deprecating,S-deprecating,G-others,S-others,General},
xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17},
xticklabels={G-b,S-b,G-re,S-re,G-f,S-f,G-t,S-t,G-r,S-r,G-d,S-d,G-o,S-o,G},
boxplot/draw direction=y,
ymin=0.6,
ymax=1,
x tick label style={rotate=90,anchor=east,font=\footnotesize},
]

\addplot[
mark=+,
very thick,
gray,
fill=gray,
boxplot
] table [row sep=\\, y index=0] {
data\\0.6959853036156031\\  0.7216471318508781\\  0.7179162301113521\\  0.704982984929509\\  0.7426968864468865\\  0.6989284448084893\\  0.7409313650424183\\  0.7097430009015375\\  0.7057364246118036\\  0.7275415401651263\\  0.7199711596842744\\  0.7118092713298959\\  0.7219597077383736\\  0.7421271936494419\\  0.6824685380603775\\  0.7161572650613413\\  0.6894031520575932\\  0.7058612119587729\\  0.7018663658916237\\  0.7108468659887691\\  0.707907620263942\\  0.7178868704052495\\  0.7077553920851022\\  0.6944976585781183\\  0.7200771614314357\\  0.7293374566925291\\  0.6965513987972048\\  0.7002404943833906\\  0.7262438980018798\\  0.7175920303144394\\  0.7241644385026738\\  0.7080891240046888\\  0.7050537994940104\\  0.7154058397259028\\  0.7025694339049932\\  0.7013927305665149\\  0.7133120957328791\\  0.6994164017645228\\  0.742791446519442\\  0.716416205745474\\  0.7001333381930397\\  0.7084142591859722\\  0.7164367275083439\\  0.699499524227785\\  0.718155922588848\\  0.7079003886587308\\  0.7141137371201233\\  0.6912674559805707\\  0.7110294431341\\  0.7099474321454864\\
};

\addplot[
mark=+,
very thick,
songcolor,
fill=songcolor,
boxplot] table [row sep=\\, y index=0] {
data\\0.7658196123701319\\  0.7659015796974016\\  0.7546718294926945\\  0.7620971902712611\\  0.7614724532954122\\  0.7772285058925887\\  0.7682846451503168\\  0.7695893934234848\\  0.7735291237176505\\  0.7806660781150111\\  0.7658942618452345\\  0.7656799130798972\\  0.7689097135058066\\  0.7611162061865688\\  0.7596658601574224\\  0.7630654188457656\\  0.7757643389996332\\  0.7620487967914439\\  0.7523424878836834\\  0.7475206611570248\\  0.7726783433679986\\  0.7876167458129395\\  0.7553844746630892\\  0.7666418946906752\\  0.7651707777000517\\  0.7711621842879234\\  0.7860431122325198\\  0.7645953581627073\\  0.7502755030594539\\  0.756324772836254\\  0.7568180987314315\\  0.771341889960157\\  0.7771809046445866\\  0.7623048180326872\\  0.7537442221602145\\  0.7678237312514093\\  0.740889785517095\\  0.776659433899191\\  0.7841781337673221\\  0.7752002782235184\\  0.7644305486991022\\  0.7725798630053949\\  0.7599231423537275\\  0.7529037434130154\\  0.7516204083368262\\  0.7654101178781926\\  0.7712020637750291\\  0.7866131784970269\\  0.7601760176017601\\  0.7507530947008964\\
};

\addplot[
mark=+,
very thick,
gray,
fill=gray,
boxplot] table [row sep=\\, y index=0] {
data\\0.7253577791827116\\  0.7142604187858376\\  0.730239116472386\\  0.7253712535806648\\  0.7037735849056603\\  0.7306940162155989\\  0.7377243161623788\\  0.7070610687022901\\  0.7291392301215484\\  0.7271502672567389\\  0.7173577913655734\\  0.7059752228986718\\  0.7367650815663662\\  0.7029151257330568\\  0.733437170937171\\  0.7387805532004319\\  0.7391372703872704\\  0.7294216373574145\\  0.7141219723183391\\  0.7602790095675132\\  0.7299729273921534\\  0.7524126395403804\\  0.6876551739027181\\  0.7399547461771468\\  0.7459299867101606\\  0.6938184066033962\\  0.7376357235501204\\  0.7427835168064377\\  0.7553346668496039\\  0.7339214570290268\\  0.7250575566824037\\  0.7293700753682768\\  0.7312285073147986\\  0.718755603370988\\  0.7195880063061784\\  0.7416690381331815\\  0.7186450044208665\\  0.7494410244497357\\  0.753728227153424\\  0.7387583856269091\\  0.7363495168391979\\  0.7641167953667953\\  0.7477123040158535\\  0.741560921075556\\  0.7635649434871224\\  0.755063715627096\\  0.7260807912382337\\  0.6888470601758722\\  0.7330352906828218\\  0.7173305899654958\\
};

\addplot[
mark=+,
very thick,
songcolor,
fill=songcolor,
boxplot] table [row sep=\\, y index=0] {
data\\0.7570492662473794\\  0.7468777924723881\\  0.7765188077688078\\  0.8003742820085232\\  0.7805244468724393\\  0.7867880211391661\\  0.772772536687631\\  0.7762464428828619\\  0.7678717141691438\\  0.782734352593377\\  0.7862032422523916\\  0.780654653561461\\  0.7806305179254388\\  0.7851714483109705\\  0.7856410256410257\\  0.787322140011383\\  0.7757317915712156\\  0.773425572519084\\  0.790546038227114\\  0.7586917876085563\\  0.7700634647487516\\  0.8030607217184754\\  0.7689502902784731\\  0.7799885924885925\\  0.7595974119338605\\  0.765727931488801\\  0.7731782699431691\\  0.7656697387258411\\  0.7547524306606525\\  0.7846976387723076\\  0.7776909722222223\\  0.792855956264347\\  0.776814171883893\\  0.7829516942064694\\  0.7734460449655074\\  0.7919777702358731\\  0.804751301956858\\  0.7881235485028975\\  0.7666424794528421\\  0.7774509803921569\\  0.7559695589901452\\  0.7652267738214831\\  0.7877697841726619\\  0.7681441635287789\\  0.8130727133887663\\  0.7646769540129393\\  0.7789332367293882\\  0.7722082833351515\\  0.7806114210217263\\  0.7813641854427863\\
};

\addplot[
mark=+,
very thick,
gray,
fill=gray,
boxplot] table [row sep=\\, y index=0] {
data\\0.7260141861622698\\  0.7794011544011544\\  0.7623756406391318\\  0.7477976190476191\\  0.7390502967822555\\  0.7404938271604938\\  0.7511980588413709\\  0.7520863570391872\\  0.7867350015073862\\  0.6964459591041869\\  0.7359484414699139\\  0.7635314995563443\\  0.7568940943174072\\  0.7932701245584681\\  0.752401313751007\\  0.7338232487115862\\  0.756839551107067\\  0.7852753415667323\\  0.7504355400696864\\  0.746072186836518\\  0.6913576555023924\\  0.7799949799196787\\  0.755327593576357\\  0.6931162148594378\\  0.7353029846246608\\  0.7701488095238095\\  0.771222929117666\\  0.7746774586173321\\  0.7494506147175862\\  0.7644256858607175\\  0.7862370087940471\\  0.7259710041166995\\  0.7375596455351057\\  0.7308396315540859\\  0.7128609422492401\\  0.7344858962693358\\  0.7865853658536586\\  0.6918958887902987\\  0.8319047619047619\\  0.7517743403093722\\  0.7445275119617225\\  0.737332853630749\\  0.7801762906997661\\  0.7596662113203064\\  0.7473958333333334\\  0.7322321428571429\\  0.8006253006253006\\  0.7799122174122174\\  0.788395061728395\\  0.714982057416268\\
};

\addplot[
mark=+,
very thick,
songcolor,
fill=songcolor,
boxplot] table [row sep=\\, y index=0] {
data\\0.7436310482668098\\  0.7854307870794407\\  0.797027600849257\\  0.7858762254901961\\  0.7896894784443774\\  0.734139341759785\\  0.800179711222656\\  0.7887891555229896\\  0.753927813163482\\  0.7717259006815969\\  0.763095238095238\\  0.7924619240408715\\  0.8099788965933072\\  0.7413397781495941\\  0.8301790281329924\\  0.7803025644179324\\  0.7866054040895814\\  0.7933641975308642\\  0.7419896640826873\\  0.7961929084753816\\  0.793859649122807\\  0.8035800677310111\\  0.7772168438557938\\  0.765586112493778\\  0.808055152394775\\  0.7919204100090443\\  0.7688880522088354\\  0.7641204127740123\\  0.732740144183932\\  0.7596596281121967\\  0.7749218374218374\\  0.7828291868026968\\  0.7885824866956942\\  0.7671943395095041\\  0.7897817649678692\\  0.8060510557831705\\  0.791846298031865\\  0.7804761904761904\\  0.8197750702905342\\  0.7351785714285715\\  0.8099788965933072\\  0.7723079819277109\\  0.7750393948944216\\  0.7677077523703291\\  0.7701220957799905\\  0.815171268679663\\  0.7641509433962265\\  0.7487962962962963\\  0.7835311481458704\\  0.8109894840415719\\
};

\addplot[
mark=+,
very thick,
gray,
fill=gray,
boxplot] table [row sep=\\, y index=0] {
data\\0.7360035211267606\\  0.7561345464571271\\  0.7006564250610029\\  0.7640134721792625\\  0.7926339285714286\\  0.7931485625753142\\  0.7875330290655778\\  0.7453472222222223\\  0.7125566275893074\\  0.7410738855255916\\  0.7963064295485636\\  0.7050888390546834\\  0.7099993034271385\\  0.721938162726056\\  0.7236141182939821\\  0.764692625082348\\  0.7175654853620955\\  0.7571203345100593\\  0.7408892000700158\\  0.7239406124342715\\  0.7419106317411402\\  0.7576215277777778\\  0.7502740476842971\\  0.6923063765736179\\  0.7029569892473119\\  0.7243395707209687\\  0.7521414755457309\\  0.6968232772252873\\  0.7260113616801515\\  0.7287633277216611\\  0.7642162944582299\\  0.7693330999474882\\  0.7529731978780209\\  0.736271303150284\\  0.7267077555213148\\  0.7306765364090205\\  0.7427061600027363\\  0.7551006341328922\\  0.7542778447237046\\  0.7405015197568389\\  0.6687673611111111\\  0.6758175766102742\\  0.7868475274725275\\  0.7207465277777778\\  0.7813696739692945\\  0.7156481322086418\\  0.7666826610001028\\  0.7082628946006555\\  0.7631181318681318\\  0.7545796952576613\\
};


\addplot[
mark=+,
very thick,
songcolor,
fill=songcolor,
boxplot] table [row sep=\\, y index=0] {
data\\0.806612114697826\\  0.7428576448676951\\  0.7878777341169106\\  0.7481283422459893\\  0.7648538737248415\\  0.7544555493430248\\  0.7776725770356344\\  0.7597736625514403\\  0.7879228375004276\\  0.779532967032967\\  0.7894890360660238\\  0.6919813902572524\\  0.7655353479152902\\  0.7661598302687411\\  0.7679219836082581\\  0.7395689416966013\\  0.7779389152921442\\  0.7822475233902036\\  0.7943665377176016\\  0.7610456299972429\\  0.7378299120234604\\  0.7354861111111111\\  0.7845220294189241\\  0.7603880494505495\\  0.7510707377728655\\  0.7882790858725762\\  0.7945398351648352\\  0.7755548662806727\\  0.7773038132080685\\  0.7525006851192108\\  0.7670400840189042\\  0.7477122390924358\\  0.7523411073526793\\  0.7855493520816101\\  0.7580623097705277\\  0.77633875106929\\  0.74024813554662\\  0.7582025185440745\\  0.7650520833333333\\  0.7371320364950938\\  0.7663667990301156\\  0.7682998922001599\\  0.7453697232317584\\  0.7697612823335168\\  0.7194159431728493\\  0.777452491011813\\  0.7587717785061239\\  0.7575237637692598\\  0.7518697441402755\\  0.7353701406120761\\
};


\addplot[
mark=+,
very thick,
gray,
fill=gray,
boxplot] table [row sep=\\, y index=0] {
data\\0.7933884297520661\\  0.6807851239669421\\  0.751984126984127\\  0.8062709966405375\\  0.6936585365853658\\  0.7209756097560975\\  0.7158730158730159\\  0.6573348264277715\\  0.7321937321937322\\  0.7010869565217391\\  0.7537593984962406\\  0.7552884615384615\\  0.6175595238095238\\  0.6993281075027995\\  0.7141500474833808\\  0.7241215574548908\\  0.7005291005291006\\  0.6932692307692307\\  0.755358807082945\\  0.7851365015166836\\  0.6170634920634921\\  0.7785114045618248\\  0.696528555431131\\  0.7105820105820105\\  0.6867724867724868\\  0.7413213885778276\\  0.6878048780487804\\  0.721875\\  0.7229268292682927\\  0.6966632962588474\\  0.6984126984126984\\  0.6728260869565217\\  0.71005291005291\\  0.7326923076923076\\  0.6741071428571429\\  0.6526794742163802\\  0.6193124368048534\\  0.7259615384615384\\  0.7708333333333334\\  0.7271825396825397\\  0.6597826086956522\\  0.6219512195121951\\  0.6884920634920635\\  0.7355324074074074\\  0.6784630940343782\\  0.6878306878306878\\  0.6663414634146342\\  0.6895661157024794\\  0.716931216931217\\  0.7789256198347108\\
};

\addplot[
mark=+,
very thick,
songcolor,
fill=songcolor,
boxplot] table [row sep=\\, y index=0] {
data\\0.7039024390243902\\  0.6430785123966942\\  0.7913533834586466\\  0.6809908998988877\\  0.8109243697478992\\  0.7149038461538462\\  0.6929563492063492\\  0.811219512195122\\  0.7878048780487805\\  0.7639029322548029\\  0.7486772486772487\\  0.734375\\  0.71005291005291\\  0.74375\\  0.7606837606837606\\  0.7932692307692307\\  0.6592261904761905\\  0.7913043478260869\\  0.7603260869565217\\  0.7663461538461539\\  0.6941463414634146\\  0.7825396825396825\\  0.7781919850885368\\  0.6978305785123967\\  0.6134615384615385\\  0.8583333333333333\\  0.7475961538461539\\  0.7992922143579373\\  0.6634615384615384\\  0.6565217391304348\\  0.7195767195767195\\  0.6585365853658537\\  0.7803921568627451\\  0.7804752066115702\\  0.7694641051567239\\  0.625\\  0.7295632698768197\\  0.7492877492877493\\  0.7505165289256198\\  0.741304347826087\\  0.7674418604651163\\  0.7481481481481481\\  0.8119312436804853\\  0.751875\\  0.7193732193732194\\  0.6725\\  0.6771739130434783\\  0.7282926829268292\\  0.7385365853658536\\  0.6750992063492064\\
};


\addplot[
mark=+,
very thick,
gray,
fill=gray,
boxplot] table [row sep=\\, y index=0] {
data\\0.7689573967030614\\  0.709542081295328\\  0.795193580057199\\  0.7558355493647376\\  0.7115515771526002\\  0.7444872618283023\\  0.7626256091775564\\  0.7220858895705522\\  0.7588876633293739\\  0.768529222864483\\  0.7724898308713337\\  0.7198857626401524\\  0.751859610123119\\  0.7378833256000338\\  0.7645990082079344\\  0.7475863821138211\\  0.7361668176133178\\  0.7104046242774567\\  0.72115506663846\\  0.7140423513175487\\  0.7482736572890025\\  0.7453164556962025\\  0.7552747204941924\\  0.7161850205198358\\  0.7502640807875945\\  0.7880909901873328\\  0.7591736244915436\\  0.7462239583333333\\  0.7172110123119015\\  0.7715561224489796\\  0.7763214531680441\\  0.7168044077134986\\  0.7509757339216019\\  0.7473641524736415\\  0.7563690169840452\\  0.7029849484187384\\  0.7581503378378378\\  0.7400393296853626\\  0.7583575581395349\\  0.7456174777603349\\  0.7517123287671232\\  0.7381825848619018\\  0.7974650912996778\\  0.7130603794312756\\  0.7843770599868161\\  0.7775788576300086\\  0.7512279810298103\\  0.7567135549872123\\  0.7526002029426687\\  0.6909256745291024\\
};


\addplot[
mark=+,
very thick,
songcolor,
fill=songcolor,
boxplot] table [row sep=\\, y index=0] {
data\\0.7637673700463201\\  0.7641287619699042\\  0.765961497778718\\  0.7450725809884636\\  0.7967687074829932\\  0.7559440559440559\\  0.7856564364876385\\  0.7506021041957156\\  0.7925897468732659\\  0.8183491403577151\\  0.743916797488226\\  0.7478298611111112\\  0.7733636977058029\\  0.8067410487018497\\  0.778337211762217\\  0.7682221283783783\\  0.7643670694209865\\  0.744166117336849\\  0.7539483206334341\\  0.7654564983888292\\  0.7619919762776906\\  0.7812282986111111\\  0.7800780587137282\\  0.7431986460757352\\  0.761808281625934\\  0.7785382231404959\\  0.7930909863945578\\  0.7478954081632653\\  0.7828231292517007\\  0.7592211357008063\\  0.773466433953429\\  0.7752557544757033\\  0.7510229046273252\\  0.7629991319444445\\  0.7616552378487946\\  0.7518367520278592\\  0.7502425443961699\\  0.7705395264587915\\  0.8311063372717508\\  0.7274119118471557\\  0.7798116035110255\\  0.8164255283249673\\  0.7831955922865014\\  0.7783599185474291\\  0.7671556013038257\\  0.7424704618689582\\  0.7754014129736673\\  0.8034651360544217\\  0.7734746307000643\\  0.7595342630853994\\
};

\addplot[
mark=+,
very thick,
gray,
fill=gray,
boxplot] table [row sep=\\, y index=0] {
data\\0.7234604779411765\\  0.6752676056338028\\  0.699009324009324\\  0.7297851129818342\\  0.7044627128596594\\  0.7640077598995778\\  0.7534911961141469\\  0.79296875\\  0.7071382007822686\\  0.6803683196918633\\  0.7724236050971174\\  0.7275482093663912\\  0.7160839160839161\\  0.7221976074435091\\  0.7196619718309859\\  0.706963249516441\\  0.745692114572635\\  0.6505089962121212\\  0.7216353677621283\\  0.7329323978171288\\  0.7130476649013\\  0.6893382352941176\\  0.7255514705882353\\  0.7394929577464788\\  0.7452356498915896\\  0.7364464962121212\\  0.7614219114219114\\  0.7455193014705882\\  0.7391608391608392\\  0.7241358901515151\\  0.7640286937405993\\  0.7396439575487846\\  0.6854875283446712\\  0.6993674662847595\\  0.7633009915769272\\  0.734525049172741\\  0.7254652193176784\\  0.7266917722241242\\  0.7045045045045045\\  0.7076056985294118\\  0.7114366197183098\\  0.7500845070422535\\  0.6975350907223553\\  0.7058857808857809\\  0.73718820861678\\  0.6964784456587735\\  0.7015269886363636\\  0.759155701754386\\  0.7273310023310023\\  0.7750863125069607\\
};

\addplot[
mark=+,
very thick,
songcolor,
fill=songcolor,
boxplot] table [row sep=\\, y index=0] {
data\\0.731638418079096\\  0.7958409926470589\\  0.7807105468314958\\  0.7324245866464723\\  0.7527777777777778\\  0.7173295454545454\\  0.7420936639118457\\  0.715619495008808\\  0.7748724489795918\\  0.7222782258064516\\  0.7666166916541729\\  0.7426900584795322\\  0.7752676056338028\\  0.7505040322580645\\  0.7611830985915493\\  0.7665107472992538\\  0.7837701612903226\\  0.780811403508772\\  0.7176596886741814\\  0.707781358157298\\  0.7376469245692114\\  0.7758501838235294\\  0.7813959358828726\\  0.7663667188315075\\  0.7492011019283746\\  0.7879818594104309\\  0.7629251700680272\\  0.7531746031746032\\  0.7724134090655975\\  0.7637293198529411\\  0.7457930540637308\\  0.6981846530794075\\  0.762995337995338\\  0.7782475490196078\\  0.755859375\\  0.6854308390022675\\  0.781859410430839\\  0.7625014918248001\\  0.8143573218761189\\  0.6357443509082853\\  0.7206866086078506\\  0.7607163828537874\\  0.7506510416666666\\  0.7301153612629022\\  0.7867030965391621\\  0.7320661157024794\\  0.7545352112676056\\  0.7462659380692167\\  0.7919274908711529\\  0.7747587316176471\\
};

\addplot[
mark=+,
very thick,
black,
fill=white,
boxplot] table [row sep=\\, y index=0] {
	data\\0.6977799168492842\\  0.7122012884301361\\  0.7212062897482866\\  0.6977416394779772\\  0.7214512378931147\\  0.708621971160993\\  0.7214591212479795\\  0.6835091620525191\\  0.7215884892135851\\  0.7075492640278679\\  0.7098960131998004\\  0.7211239520754845\\  0.7203640492804243\\  0.7031084088867108\\  0.6996443299719902\\  0.6823407263069797\\  0.696287228549188\\  0.6871266111982541\\  0.7161420911413423\\  0.6931013368711093\\  0.6986271378528746\\  0.7021834938466339\\  0.7188209341322264\\  0.7137679584568064\\  0.681357919557003\\  0.700979475820391\\  0.7095922304149992\\  0.7141676871789638\\  0.7031876197240696\\  0.7067981187703007\\  0.6918972700176128\\  0.6905701754385964\\  0.6839524282960523\\  0.7063027539364901\\  0.6978813123521547\\  0.6972927909581509\\  0.7032434734415483\\  0.690907784948284\\  0.6933421499869367\\  0.6812814105552202\\  0.7082526733830761\\  0.7119489435189816\\  0.7104448727859836\\  0.6878634441852352\\  0.6947641803093637\\  0.7265286409026567\\  0.6900298144359712\\  0.6992096877644041\\  0.6905252869999562\\  0.7201383278404014\\
};

\end{axis}
\end{tikzpicture}
}

==> figure/correctness.tex <==
\scalebox{0.5}{
\begin{tikzpicture}
\pgfplotsset{
	   boxplot/every whisker/.style={thick,solid,black},
	   boxplot/every median/.style={very thick,solid,black},
	   %boxplot/every box/.style={very thick,solid,draw=black},
}
\begin{axis}[
xtick={1,2},
xticklabels={ \small 
\texttt{PyEvosuite},{\tool}
},
boxplot/draw direction=y,
ymin= 1,
ymax= 5,
%x tick label style={rotate=0,anchor=east},
%cycle list={{red},{blue},{green}},
]



\addplot[
very thick,
mark=+,
fill=gray,
boxplot
]
table [row sep=\\, y index=0] {
	data\\0.2\\0.33\\0.25\\0.1\\0\\0.4\\0.25\\
};

\addplot[
very thick,
mark=+,
boxplot] 
table [row sep=\\, y index=0] {
data\\0.33\\.25\\0.4\\0.1\\0.6\\0.2\\0.4\\
};

\end{axis}
\end{tikzpicture}
}

==> figure/pgfplots/overlap.tex <==
\begin{figure}[t!]
\centering
\footnotesize
%\scalebox{0.8}{
	\begin{tikzpicture}[thick, scale=0.85]
	\begin{axis}[
	ybar stacked,
	height=3.8cm,
	width=9.5cm,
	enlargelimits=0.2,
	legend style={at={(0.5, -0.23)}, anchor=north, legend columns=-1},
	ymin= 0,
	%ylabel={\#Reviewers involved},
	%xtick={CompanyX, Qt, Android, Openstack},
	symbolic x coords={Microsoft, Qt, Android, OpenStack},
	xtick=data,
	x tick label style={font=\footnotesize},
	%nodes near coords,
	%nodes near coords align = {vertical},
	]
\addplot+[ybar,gray,  fill=gray]coordinates{(Microsoft, 0.913) (Qt,0.837) (Android, 0.844) (OpenStack,0.806)};
\addplot +[ybar, gray!50, fill=gray!50]coordinates{(Microsoft, 0.08) (Qt,0.1136) (Android,0.136) (OpenStack,0.16)};
\addplot +[ybar, gray!75, fill=gray!75]coordinates{(Microsoft, 0.006) (Qt,0.05) (Android,0.018) (OpenStack,0.029)};
\addplot +[ybar, gray!90, fill=gray!90]coordinates{(Microsoft, 0.0002) (Qt,0.0001) (Android,0.003) (OpenStack,0.005)};
\legend{2 intents, 3 intents, 4 intents, 5 intents}

\end{axis}
\end{tikzpicture}
%}
\vspace{-0.1in}
\caption{\small The distribution of changes with multiple change intents.}
\label{fig:overlaps}
\vspace{-0.1in}
\end{figure}


==> figure/pgfplots/pie.tex <==
\begin{tikzpicture}
\pie[text=pin, color ={black!3, black!10, black!20, black!30, black!40, black!50, 
black!55, black!60, black!65, black!70}]
{40/Bug Fix \& Resource, 14/Bug Fix \& Test, 12/Deprecate \& Resource, 
12/Test \& Resource, 5/Merge \& Resource, 5/Bug Fix \& Deprecate,
4/Bug Fix \& Feature, 3/Test \& Deprecate, 
3/Bug Fix \& Refactor, 2/Feature \& Resource}
\end{tikzpicture}


==> figure/pgfplots/reviewer.tex <==
\begin{figure}[t!]
\centering
\footnotesize
%\scalebox{0.8}{
	\begin{tikzpicture}[thick, scale=0.8]
	\begin{axis}[
	ybar,
	height=3.8cm,
	width=9.5cm,
	enlargelimits=0.2,
	legend style={at={(0.8, 0.93)}, anchor=north, legend columns=1},
	ymin= 0,
	ylabel={\#Reviewers involved},
	%xtick={CompanyX, Qt, Android, Openstack},
	symbolic x coords={CompanyX, Qt, Android, OpenStack},
	xtick=data,
	x tick label style={font=\footnotesize},
	%nodes near coords,
	%nodes near coords
	%align={vertical},
	]
\addplot+[ybar,gray,  fill=gray]coordinates{(CompanyX, 4.8) (Qt,3.1) (Android,2.5) (OpenStack,2.5)};
\addplot +[ybar, gray!25, fill=gray!25]coordinates{(CompanyX, 6.23) (Qt,3.6) (Android,3.1) (OpenStack,3.0)};
\legend{Regular, LRE}

\end{axis}
\end{tikzpicture}
%}
\vspace{-0.1in}
\caption{\small Average \#reviewers involved for reviewing changes.}
\label{fig:avg_reviewer}
\end{figure}


==> figure/pgfplots/select_features.tex <==
\begin{figure}[t!]
\centering
\footnotesize

\begin{tikzpicture}[thick, scale=0.85]
\begin{axis}[
ybar stacked,
height=3.8cm,
width = 9cm,
enlargelimits=0.15,
legend style={at={(0.5,-0.22)},
	anchor=north,legend columns=-1},
%ylabel={\#participants},
symbolic x coords={Microsoft, Qt, Android, OpenStack, Together},
xtick=data,
x tick label style={font=\footnotesize},
]
\addplot+[ybar,gray,  fill=gray] plot coordinates {(Microsoft,0.60) (Qt,0.24)
	(Android,0.21) (OpenStack,0.44) (Together,0.77)};
\addplot+[ybar, gray!25, fill=gray!25] plot coordinates {(Microsoft,0.40) (Qt,0.76) 
	(Android,0.79) (OpenStack,0.56) (Together,0.23)};
%\addplot+[ybar] plot coordinates {(tool1,6) (tool2,6)
%(tool3,8) (tool4,2) (tool5,6) (tool6,5) (tool7,6)};
%\addplot+[ybar] plot coordinates {(tool1,4) (tool2,2)
%(tool3,0) (tool4,2) (tool5,3) (tool6,2) (tool7,4)};
\legend{correlated, uncorrelated}
\end{axis}
\end{tikzpicture}
\vspace{-0.1in}
\caption{\small The distributions of correlated and uncorrelated features
in each project and across the projects (i.e., Together).}
\label{fig:s_feature}
\vspace{-0.1in}
\end{figure}


==> figure/pgfplots/sfeature.tex <==
\begin{tikzpicture}[thick, scale=0.85]
\begin{axis}[
ybar stacked,
height=3.8cm,
width = 9cm,
enlargelimits=0.15,
legend style={at={(0.5,-0.22)},
anchor=north,legend columns=-1},
%ylabel={\#participants},
symbolic x coords={CompanyX, Qt, Android, OpenStack, Together},
xtick=data,
x tick label style={font=\footnotesize},
]
\addplot+[ybar,gray,  fill=gray] plot coordinates {(CompanyX,0.60) (Qt,0.24)
(Android,0.21) (OpenStack,0.44) (Together,0.77)};
\addplot+[ybar, gray!25, fill=gray!25] plot coordinates {(CompanyX,0.40) (Qt,0.76) 
(Android,0.79) (OpenStack,0.56) (Together,0.23)};
%\addplot+[ybar] plot coordinates {(tool1,6) (tool2,6)
%(tool3,8) (tool4,2) (tool5,6) (tool6,5) (tool7,6)};
%\addplot+[ybar] plot coordinates {(tool1,4) (tool2,2)
%(tool3,0) (tool4,2) (tool5,3) (tool6,2) (tool7,4)};
\legend{correlated, uncorrelated}
\end{axis}
\end{tikzpicture}



==> figure/pgfplots/time.tex <==
\begin{figure}[t!]
\centering
\footnotesize
%\scalebox{0.8}{
	\begin{tikzpicture}[thick, scale=0.8]
	\begin{axis}[
	ybar,
	height=3.8cm,
	width=9.5 cm,
	enlargelimits=0.2,
	legend style={at={(0.8, 0.93)}, anchor=north, legend columns=1},
	ymin=0,
	ylabel={Review duration (h)},
	%xtick={CompanyX, Qt, Android, Openstack},
	symbolic x coords={CompanyX, Qt, Android, OpenStack},
	xtick=data,
	x tick label style={font=\footnotesize},
	%nodes near coords,
	%nodes near coords
	%align={vertical},
	]
\addplot+[ybar,gray,  fill=gray]coordinates{(CompanyX, 43.7) (Qt,45.0) (Android,92.8) (OpenStack,45.5)};
\addplot +[ybar, gray!25, fill=gray!25]coordinates{(CompanyX, 169) (Qt,189.4) (Android,910.4) (OpenStack,172.9)};
\legend{Regular, LRE}

\end{axis}
\end{tikzpicture}
%}
\vspace{-0.1in}
\caption{\small Average review durations for \emph{regular} and \emph{LRE changes}.}
\label{fig:avg_times}
\end{figure}


==> figure/readability.tex <==
\scalebox{0.5}{
\begin{tikzpicture}
\pgfplotsset{
	   boxplot/every whisker/.style={thick,solid,black},
	   boxplot/every median/.style={very thick,solid,black},
	   %boxplot/every box/.style={very thick,solid,draw=black},
}
\begin{axis}[
xtick={1,2,3},
xticklabels={\texttt{PyEvosuite},,\texttt{Mutester}},
boxplot/draw direction=y,
ymin= 0,
ymax= 6,
%x tick label style={rotate=0,anchor=east},
%cycle list={{red},{blue},{green}},
]



\addplot[
very thick,
mark=+,
fill=gray,
boxplot
]
table [row sep=\\, y index=0] {
	data\\2\\3\\2.5\\1\\3\\2\\2.5\\3\\4\\2.5\\3\\2\\1\\3\\2.5\\
};

\addplot[
very thick,
mark=+,
fill=white,
boxplot
]
table [row sep=\\, y index=0] {
	data\\0\\
};

\addplot[
very thick,
mark=+,
boxplot] 
table [row sep=\\, y index=0] {
data\\3\\4.5\\4\\2\\5\\2.5\\3.5\\3\\4\\5\\4.5\\3.5\\2.5\\4\\4.5\\3\\
};

\end{axis}
\end{tikzpicture}
}


==> figure/usefulness.tex <==
\scalebox{0.5}{
\begin{tikzpicture}
\pgfplotsset{
	   boxplot/every whisker/.style={thick,solid,black},
	   boxplot/every median/.style={very thick,solid,black},
	   %boxplot/every box/.style={very thick,solid,draw=black},
}
\begin{axis}[
xtick={1,2,3},
xticklabels={\texttt{PyEvosuite},,\texttt{Mutester}},
boxplot/draw direction=y,
ymin= 0,
ymax= 6,
%x tick label style={rotate=0,anchor=east},
%cycle list={{red},{blue},{green}},
]



\addplot[
very thick,
mark=+,
fill=gray,
boxplot
]
table [row sep=\\, y index=0] {
	data\\2\\3\\2\\1\\2\\2\\2.5\\3\\2\\2\\3\\2.5\\1\\3\\2\\
};

\addplot[
very thick,
mark=+,
fill=white,
boxplot
]
table [row sep=\\, y index=0] {
	data\\0\\
};

\addplot[
very thick,
mark=+,
boxplot] 
table [row sep=\\, y index=0] {
data\\3.5\\5\\4\\2.5\\3.5\\4.5\\4.5\\3.5\\5\\4\\4.5\\3.5\\3\\4\\5\\3.5\\
};

\end{axis}
\end{tikzpicture}
}

==> sec/Patterntable.tex <==
% \begin{table*}[t!]
% \caption{Patterns for mining API constraints.\song{Nima: please correct the format of rules, and also add a column to show the id}}
% 	\label{tab:patterns}
% 	\setlength{\tabcolsep}{3pt} 
% 	\scalebox{0.9}{
% \begin{tabular}{ll}
% \toprule
% Rules & Example Sentences \\ \midrule
% \textless{}D\_type\small default=\textless{}value\small{} & int default=0 \\
% \textless{}D\_type\small or \textless{}D\_type\small{} & int or float \\
% \textless{}Structure\small of shape \textless{}(shape)\small{}, default=\textless{}value\small{} & array-like of shape (n\_samples,n\_features), default=None \\
% \textless{}Structure\_Enum\small of shape \textless{}(shape)\small{}, default=\textless{}value\small{} & \{array-like, sparse matrix\} of shape (n\_samples, n\_features), default=None \\
% \textless{}Structure\small of shape \textless{}(shape)\small or \textless{}(shape)\small{} & array-like of shape (n\_samples,n\_features) or (n\_samples,) \\
% \textless{}D\_type\small{}/\textless{}structure\small{} & params: dict \\
% \{Structure\_Enum\} & \{list, tuple, set\} \\
% \{Values\_Enum\} default=\textless{}value\small{} & \{‘text’, ‘diagram’\}, default=None \\
% \{Values\_Enum\} & \{‘text’, ‘diagram’\} \\
% \textless{}Size\small length of \{Structure\_Enum\} & 2-length sequence (tuple, list, …) \\
% \textless{}Dimension\small d \textless{}structure\small{} & 2d Array \\
% \textless{}value\small (def), \textless{}value\small{},.... or \textless{}value\small{} & ‘backward’ (default), ‘forward’, or ‘nearest’ \\
% \textless{}Structure\small of  \textless{}D\_type\small{} & tuple of ints \\
% \textless{}value\small or \textless{}value\small{} & \cellcolor[HTML]{FFFFFF}None or "sequence" \\
% \textless{}D\_type\small{},optional & (int,optional) \\
% \textless{}Structure\small{},optional & (array-like,optional) \\
% \textless{}D\_type\small or \textless{}value\small{} & int or “all” \\
% \cellcolor[HTML]{FFFFFF}\textless{}D\_type\small or \textless{}value\small default=\textless{}value\small{} & int or “all”, default=10 \\ \bottomrule
% \end{tabular}
% }
% \end{table*}


\begin{table*}[t!]
\caption{Rules for mining constraints from parametric pages of APIs.\song{add a new column between "No" and "Rules", group them into different types, i.e., structure, shape, data type, default value, and optionality}}
\label{tab:ruless}%\arun{Unlike that related paper , our designed rule can get all the constraints in a parametric sentence using one rule alone, so we cant group them based on each constraint.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
\toprule
No & Rules & Examples                   \\
\midrule
1 &  & \textless{}D\_type\textgreater \, default=\textless{}value\textgreater{} & int default=0                       \\
2  & \textless{}D\_type\textgreater \, or \textless{}D\_type\textgreater{}    & int or float                        \\
3 &
  \textless{}Structure\textgreater \, of shape \textless{}(shape)\textgreater{}, default=\textless{}value\textgreater{} &
  array-like of shape (n\_samples,n\_features), default=None \\
4 &
  \textless{}Structure\_Enum\textgreater \, of shape \textless{}(shape)\textgreater{}, default=\textless{}value\textgreater{} &
  \{array-like, sparse matrix\} \, of shape (n\_samples, n\_features), default=None \\
5 &
  \textless{}Structure\textgreater \, of shape \textless{}(shape)\textgreater \, or \textless{}(shape)\textgreater{} &
  array-like of shape (n\_samples,n\_features) \, or (n\_samples,) \\
6  & \textless{}D\_type\textgreater{}/\textless{}structure\textgreater{}   & params: dict                        \\
7  & \{Structure\_Enum\}                                                   & \{list, tuple, set\}                \\
8  & \{Values\_Enum\} default=\textless{}value\textgreater{}               & \{`text', `diagram'\}, default=None \\
9  & \{Values\_Enum\}                                                      & \{`text', `diagram'\}               \\
10 & \textless{}Size\textgreater length of \{Structure\_Enum\}             & 2-length sequence (tuple, list, …)  \\
11 & \textless{}Dimension\textgreater \, d \textless{}structure\textgreater{} & 2d Array                            \\
12 &
  \textless{}value\textgreater (def), \textless{}value\textgreater{}, .... or \textless{}value\textgreater{} &
  `backward' (default), `forward', or `nearest' \\
13 & \textless{}Structure\textgreater \, of \textless{}D\_type\textgreater{}  & tuple of ints                       \\
14 & \textless{}value\textgreater \, or \textless{}value\textgreater{}        & None or ``sequence''                  \\
15 & \textless{}D\_type\textgreater{}, optional                             & (int,optional)                      \\
16 & \textless{}Structure\textgreater{}, optional                           & (array-like,optional)               \\
17 & \textless{}D\_type\textgreater \, or \textless{}value\textgreater{}      & int or ``all''                        \\
18 &
  \textless{}D\_type\textgreater \, or \textless{}value\textgreater default=\textless{}value\textgreater{} & 
  int or ``all'', default=10 \\
  \bottomrule
\end{tabular}}
\end{table*}





==> sec/code/MUT_code.tex <==
\begin{lstlisting}[language=Python]
import k_means as module_0
import _split as module_1

def test_case_2():
    int_0 = 19
    var_0 = module_0.KMeans(int_0)
    float_0 = 1.6484
    int_2 = 69672
    float_1 = 83.14
    int_3 = 5568
    list_0 = [[float_0,int_2],[float_1,int_3]]
    var_1 = module_1.train_test_split(list_0)
    var_2 = var_0.fit(list_0)
    var_3 = var_0.predict(list_0)

\end{lstlisting}

==> sec/dv.tex <==
\section{Data Availability}
The source code of {\tool} and the dataset of our experiment artifacts
are available on Zenodo~\cite{anonymous_2023_7608421}.

==> table/RQ3.tex <==
\begin{table}[t!]
\caption{Code coverage results for test cases generated by {\tool} and the improvement to \textbf{PyEvosuite}.}
\label{mutestResult2}
%\song{show the number of tests generated, and the improvement to the best coverage from either PyEvosuite or PyRandoop}}
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Framework}} & \multicolumn{3}{c|}{{\tool}}                   \\ \cline{2-4} 
& \multicolumn{1}{l|}{\textbf{\#Test}} & \textbf{Coverage} &\textbf{Improvement} \\ \hline
 Scikit-Learn & \multicolumn{1}{l|}{1588}                & \multicolumn{1}{l|}{62.59\%}  & 27.00\%              \\ \hline
% Pandas& \multicolumn{1}{l|}{697}                &    \multicolumn{1}{l|}{68.17\%}  &  18.0\%            \\ \hline
% Numpy& \multicolumn{1}{l|}{1143}                &   \multicolumn{1}{l|}{56.23\%}   &  41.9\%              \\ \hline
% Scipy & \multicolumn{1}{l|}{633}                &  \multicolumn{1}{l|}{51.19\%}   & 22.5\%                \\ \hline
 PyTorch & \multicolumn{1}{l|}{529}                &  \multicolumn{1}{l|}{32.97\%}  &  18.60\%              \\ \hline 
 TensorFlow & \multicolumn{1}{l|}{661}                &  \multicolumn{1}{l|}{29.12\%}  &   20.98\%             \\ \hline
 CNTK & \multicolumn{1}{l|}{318}                &  \multicolumn{1}{l|}{41.07\%}  &  15.72\%             \\ \hline
\end{tabular}
\end{table}

==> table/parameterPage.tex <==
    \begin{table}[t!]
\begin{tabular}{|l|l|}
\multirow{6}{*}{\textbf{Parameters:}} & \textit{\textbf{X: \{array-like, sparse matrix\} of shape (n\_samples, n\_features)}}  \\
  & \begin{tabular}[c]{@{}l@{}}Training instances to cluster. It must be noted that the data will be converted to C ordering, \\ which will cause a memory copy if the given data is not C-contiguous. If a sparse matrix \\ is passed, a copy will be made if it’s not in CSR format.\end{tabular} \\
 & \textit{\textbf{y: Ignored}}                                                           \\
   & Not used, present here for API consistency by convention.                              \\
    & \textit{\textbf{sample\_weight: array-like of shape (n\_samples,), default=None}}      \\
    & The weights for each observation in X. If None, all observations are assigned equal weight.  
\end{tabular}
\end{table}                                                       
